On $f$-divergences between Cauchy distributions

We prove that the $f$-divergences between univariate Cauchy distributions are all symmetric, and can be expressed as strictly increasing scalar functions of the symmetric chi-squared divergence. We report the corresponding scalar functions for the total variation distance, the Kullback-Leibler divergence, the squared Hellinger divergence, and the Jensen-Shannon divergence among others. Next, we give conditions to expand the $f$-divergences as converging infinite series of higher-order power chi divergences, and illustrate the criterion for converging Taylor series expressing the $f$-divergences between Cauchy distributions. We then show that the symmetric property of $f$-divergences holds for multivariate location-scale families with prescribed matrix scales provided that the standard density is even which includes the cases of the multivariate normal and Cauchy families. However, the $f$-divergences between multivariate Cauchy densities with different scale matrices are shown asymmetric. Finally, we present several metrizations of $f$-divergences between univariate Cauchy distributions and further report geometric embedding properties of the Kullback-Leibler divergence.

==> macroFdivCauchy.tex <==

\def\leftsup#1{{}^{#1}}
\def\calLC{\mathcal{LC}}
\def\lc{\mathrm{lc}}
\def\wc{\mathrm{wc}}
\def\HM{\mathrm{HM}}
\def\JS{\mathrm{JS}}
\def\TV{\mathrm{TV}}
\def\LC{\mathrm{LC}}
\def\BC{\mathrm{BC}}
\def\Bhat{\mathrm{Bhat}}
\def\dz{\mathrm{d}z}
\def\Im{\mathrm{Im}}
\def\Re{\mathrm{Re}}
\def\FR{\mathrm{FR}}
\def\SL{\mathrm{SL}}
\def\SU{\mathrm{SU}}
\def\KC{\mathrm{KC}}
\def\bbC{\mathbb{C}}
\def\bbU{\mathbb{U}}
\def\bbD{\mathbb{D}}
\def\calLN{\mathcal{LN}}
\def\calG{\mathcal{G}}
\def\calL{\mathcal{L}}
\def\calH{\mathcal{H}}
\def\GL{\mathrm{GL}}
\def\arccosh{\mathrm{arccosh}}
\def\sech{\mathrm{sech}}
\def\dl{\mathrm{d}l}
\def\ds{\mathrm{d}s}
\def\dlambda{\mathrm{d}\lambda}
\def\dtheta{\mathrm{d}\theta}
\def\JS{\mathrm{JS}}
\def\MI{\mathrm{MI}}
\def\elliptical{\mathrm{ell}}
\def\calM{\mathcal{M}}
\def\normal{\mathcal{N}}
\def\Rayleigh{\mathrm{Rayleigh}}
\def\Cauchy{\mathrm{Cauchy}}
\def\Mah{\mathrm{Mah}}
\def\IS{\mathrm{IS}}
\def\diag{\mathrm{diag}}
\def\calE{\mathcal{E}}
\def\calR{\mathcal{R}}
\def\calL{\mathcal{L}}
\def\calN{\mathcal{N}}
\def\calC{\mathcal{C}}
\def\calS{\mathcal{S}}
\def\calK{\mathcal{K}}
\def\calP{\mathcal{P}}
\def\calQ{\mathcal{Q}}
\def\LS{\mathrm{LS}}
\def\tr{\mathrm{tr}}	
\def\bbP{\mathbb{P}}
\def\eqdef{:=}
\def\hcross{{h^\times}}
\def\hcrossent#1#2{{\hcross}\left(#1:#2\right)}
\def\arctanh{\mathrm{arctanh}}
\def\dmu{\mathrm{d}\mu}
\def\bbH{\mathbb{H}}
\def\dx{\mathrm{d}x}
\def\dy{\mathrm{d}y}
\def\KL{\mathrm{KL}}
\def\kl{\mathrm{kl}}
\def\bbR{{\mathbb{R}}}
\def\calF{\mathcal{F}}
\def\calX{\mathcal{X}}
\def\calY{\mathcal{Y}}
\def\st{\ :\ }
\def\SO{\mathrm{SO}}
\def\Jac{\mathrm{Jac}}
\def\equaldist{\stackrel{d}{=}}
\def\bbG{\mathbb{G}}
\def\mattwotwo#1#2#3#4{\left[\begin{array}{cc}#1 & #2\\ #3 & #4\end{array}\right]}
\def\Sym{\mathrm{Sym}}
\def\cc{\mathrm{cc}}
\def\Cauchy{\mathrm{Cauchy}}
\def\CCauchy{\mathrm{CCauchy}}
\def\WCauchy{\mathrm{WCauchy}}
\def\LogCauchy{\mathrm{LogCauchy}}
